Path ORAM: An Extremely Simple Oblivious RAM Protocol

We present Path ORAM, an extremely simple Oblivious RAM protocol with a small amount of client storage. Partly due to its simplicity, Path ORAM is the most practical ORAM scheme known to date with small client storage. We formally prove that Path ORAM has a O(log N) bandwidth cost for blocks of size B = Omega(log^2 N) bits. For such block sizes, Path ORAM is asymptotically better than the best known ORAM schemes with small client storage. Due to its practicality, Path ORAM has been adopted in the design of secure processors since its proposal.

==> Chernoff.tex <==
\subsection{Details of Chernoff Bound}\label{app:Chernoff}



\begin{figure}[t]
\centering
\includegraphics[width=0.77\columnwidth]{Figures/ProofTree}
\caption{Subtree $T$ for proof in Section~\ref{app:Chernoff}.}
\label{fig:ProofTree}
\end{figure}


Before getting into proof details, we start by giving some intuition on how blocks get evicted from a subtree $T$ in $\infty$-ORAM. For simplicity we assume $T$ has no leafs with the ORAM tree in common. Figure \ref{fig:ProofTree} gives an example of a subtree $T$; the figure also shows the boundary nodes that are at one edge distance from $T$. When blocks get evicted from $T$, they will pass through one of these boundary nodes to a higher level outside $T$.  $X_1$ is the most recent label of a block that was read from ORAM and written back with a new random label $Y_1$. $X_2$ is the next older label of a block that was read from ORAM and written back with a new random label $Y_2$, etc. 

We define $S_j$ as the set of leafs of the ORAM tree that can be reached through a path that has a boundary node in common with one of the paths to $X_1$, $X_2$, $\ldots$, or $X_j$. In the example: $|S_1|<|S_2|$, since $X_1$ and $X_2$ have no boundary point in common; $S_2=S_3$, since $X_3$ and $X_1$ have a boundary point in common; $S_3=S_4$, since $X_4$ and $X_2$ have a boundary point in common; $|S_4|<|S_5|$, since $X_5$ has no boundary point in common with $S_4$.

Notice that the block with label $Y_j$ only gets evicted if it is in $S_j$, i.e., one of the more recent load/stores of a path to$X_i$, $1\leq i\leq j$, has a boundary node in common with the path to $Y_j$ over which the corresponding block will get evicted from $T$. We introduce the following notation: $w_1=|S_1|< w_2=|S_2|=|S_3|=|S_4|<w_3=|S_5|\ldots$ and $q_1=1$ denoting the number of sets $S_j$ with size equal to $w_1$, $q_2=3$ denoting the number of sets $S_j$ with size equal to $w_2$ etc. Let $m_1=I(Y_1\not\in S_1)$, $m_2= I(Y_2\not\in S_2)+I(Y_3\not\in S_3)+I(Y_4\not\in S_4)$, where $I(.)$ is the indicator function outputting 1 if the input is true and 0 if the input is false. We are interested in the sum $M=\sum_j m_j$, which is the number of blocks not evicted from $T$, in other words it equals the usage of $T$.

The probability distribution of $q_i$ is a geometric distribution with its parameter a function of $w_i$. The probability distribution of $m_i$ is a binomial distribution with its parameters characterized by $q_i$ and $w_i$. The probability distribution of $w_i$ is not correlated with $q_i$ and $m_i$. These dependencies allow us to use Bayes rule to compute the probability distribution on $M$. The proof now proceeds by only considering the worst case sequence $(w_i)_{i\geq 1}$ and use probability generating functions to upper bound the tail distribution of $M$ by using Chernoff bounding techniques. 

We will now prove in detail an upper bound on the probability in the sum of the right-hand side of (\ref{equnion}) for general $T$ with $n(T)=n$. To this purpose
let $\mbox{{\bf a}}=(a_j)_{j=1}^s$ be a sequence of block addresses with working set size $N$, i.e., $\mbox{{\bf a}}$ has $N$ different block addresses.
 
\vspace{.2cm}

\noindent
{\bf Worst-case address pattern.} In $\infty$-ORAM a worst-case address pattern $\mbox{{\bf a}}$ for a fixed working set size $N$ does not duplicate block addresses, i.e., $s=N$ and as a consequence the labels in $(X_j)_{j=1}^N$ and $(Y_j)_{j=1}^N$ (that define $\mbox{{\bf s}}$ given $a(\mbox{{\bf s}})=\mbox{{\bf a}}$) are all statistically independent of one another:

Suppose that there exists an address in $\mbox{{\bf a}}$ that has been loaded/stored twice in $\infty$-ORAM.
Then, there exist indices $i$ and $j$, $i<j$, with $a_i=a_j$. Without the $j$-th load/store, the working set remains the same  and it is more likely for older blocks corresponding to $a_k$, $k>j$ to {\em not} have been evicted from $T$ (since there is one less load/store that could have evicted an older block to a higher level outside $T$; also notice that buckets in $\infty$-ORAM are infinitely sized, so, removing the $j$-th load/store does not generate extra space that can be used for storage of older blocks that otherwise would not have found space). So, to maximize the probability of the right-hand side of (\ref{equnion}), we may assume that $\mbox{{\bf a}}=(a_j)_{j=1}^s$ is a sequence of block addresses without duplicates.


\vspace{.2cm}

\noindent
{\bf Blocks that remain in $T$ with probability $1$.} Let $V$ be the set of  leafs in $T$ that are also leafs in the ORAM tree. Notice that if a block corresponds to a $Y_j\in V$, then it never gets evicted from $T$ since the whole path to the leaf with label $Y_j$ is part of $T$. The probability that $m_0$ out of the $N$ labels $Y_j$ are in $V$ is equal to the binomial
\begin{equation}
p_0 = Prob(m_0) = {N \choose m_0} (\frac{|V|}{2^L})^{m_0} (1-\frac{|V|}{2^L})^{N-m_0}.\label{eqp1}
\end{equation}
$T$'s usage in (\ref{equnion}) is {\em upper bounded} by the number $m_0$ of $Y_j$'s that are in $V$ added to $T$'s usage after an {\em infinite} sequence of load/store operations, where (1) all $Y_j\not\in V$ (those $Y_j$ that were in $V$ are replaced by labels not in $V$ and the sequence is extended with labels not in $V$) and (2) labels $X_j$ and $Y_j$ are uniformly distributed and statistically independent.

In (\ref{equnion}) we are only interested in a non-zero probability that $T$'s usage is $>nZ+R$. 
Therefore, without loss of generality, 
we may constrain $|V|$ to lead to such a non-zero probability. 
Since $|V|\leq n$ and $T$'s usage is at most the number $N$ of different blocks, we may assume $|V|Z\leq nZ+R\leq N$, hence,
\begin{equation} |V|\leq N/Z. \label{alpha} \end{equation}


\noindent
{\bf Block eviction from $T$.} Consider the infinite sequence of load/store operations. For each leaf label $X$ we define $X(T)$ as the set of leafs that can be reached from a bucket $b\not\in T$ that is on the path from the root to $X$. Notice that $X(T)=\emptyset$ if and only if $X\in V$. Furthermore, the number of different non-empty sets $X(T)$ is equal to the number of nodes in the ORAM tree that are one edge away from $T$:
\begin{equation}
\# \mbox{ distinct non-empty sets } X(T) = 1+n-2|V|. \label{eqset}
\end{equation}
The non-empty sets $X(T)$ do not intersect with $V$.

By the definition of $X_i(T)$, if $\infty$-ORAM reads/writes a path to $X_i$ and $Y_j\in X_i(T)$ for $j\geq i$, then $Y_j$ gets written to a bucket outside $T$:
The block corresponding to $Y_j$ is counted in $T$'s usage if and only if $Y_j \not\in S_j = \cup_{i=1}^j X_i(T).$

\vspace{.2cm}

\noindent
{\bf Eviction probability as a function of the sizes $|S_j|$.}
The sizes of sets $S_j$ are uniquely determined by the sequence 
$$w_1=|S_1|=\ldots =|S_{q_1}|, \ w_2=|S_{q_1+1}|=\ldots =|S_{q_1+q_2}|, \mbox{ etc.} $$
By (\ref{eqset}), the number of $w_j$ is at most $1+n-2|V|$ and if $w_{1+n-2|V|}$ exists, then its is equal to $2^L-|V|$. 

Let $m_k$ be equal to the number of blocks in the subsequence $(Y_{(\sum_{t=1}^{k-1} q_t) + 1}, \ldots,  Y_{\sum_{t=1}^{k} q_t })$ that are $\not\in S_{\sum_{t=1}^{k-1} q_t + 1}= \ldots =S_{\sum_{t=1}^{k} q_t }$, in other words, they do not get evicted from $T$. Since leaf labels $Y_j$ are $\not\in V$, the probability that $Y_j\not\in S_j$ is equal to $1-|S_j|/(2^L-|V|)$, hence, 
\begin{eqnarray}
&& Prob(m_k | (w_t,q_t,m_t)_{t=1}^{k-1},w_k,q_k)  = Prob(m_k | w_k,q_k) \nonumber \\
&& = {q_k \choose m_k} (1-\frac{w_k}{2^L-|V|})^{m_k} (\frac{w_k}{2^L-|V|})^{q_k-m_k}. \label{eqp2}
\end{eqnarray}
Probability (\ref{eqp2}) is zero for $k\geq 1+n-2|V|$, so we may restrict $k$ to $\leq n-2|V|$.

Since leaf labels $X_j$ are not constrained, the probability that $S_j$ has size $|S_j|=|S_{j-1}|$ is equal to $(|S_{j-1}|+|V|)/2^L$, the probability that $X_j\in S_{j-1}\cup V$. Hence,
\begin{eqnarray}
&& Prob(q_k | (w_t,q_t,m_t)_{t=1}^{k-1},w_k)= Prob(q_k | w_k) \nonumber \\
&&  = (\frac{w_k+|V|}{2^L})^{q_k-1}(1-\frac{w_k+|V|}{2^L}).\label{eqp3}
\end{eqnarray}

The probability that $w_k$ takes on a certain value only depends on the previous values  $w_t$, $t<k$, since they determine the sizes of previously added $X_j(T)$s and therefore determine the sizes of sets $X_j(T)$ that can still be added to $S_{k-1}$:
\begin{equation}
Prob(w_k|(w_t,q_t,m_t)_{t=1}^{k-1}) = Prob(w_k | (w_t)_{t=1}^{k-1}).\label{eqp4}
\end{equation}

We combine (\ref{eqp2}), (\ref{eqp3}) and (\ref{eqp4}) by using Bayes rule twice:
\begin{eqnarray*}
&& Prob((w_t,q_t,m_t)_{t\geq 1}) \\
&& = \prod_{k\geq 1 } Prob(m_k | w_k,q_k)Prob(q_k | w_k)Prob(w_k | (w_t)_{t=1}^{k-1}) \\
&& = Prob((w_t)_{t\geq 1})  \prod_{k\geq 1 } Prob(m_k | w_k,q_k)Prob(q_k | w_k).
\end{eqnarray*}
If we sum over all possible sequences $(w_t,q_t)_{t\geq 1}$ we obtain
\begin{eqnarray*}
&& Prob((m_t)_{t\geq 1}) \\ 
&& = \sum_{(w_t,q_t)_{t\geq 1}} Prob((w_t)_{t\geq 1}) \cdot \\
&& \hspace{.5cm} \cdot \prod_{k\geq 1 } Prob(m_k | w_k,q_k)Prob(q_k | w_k) \\
&& = \sum_{(w_t)_{t\geq 1}} Prob((w_t)_{t\geq 1})  \cdot \\
&& \hspace{.5cm} \cdot \prod_{k\geq 1 } \sum_{q\geq 1} Prob(m_k | w_k,q_k=q)Prob(q_k=q | w_k).
\end{eqnarray*}
Substituting (\ref{eqp2}) and (\ref{eqp3}) yields
\begin{eqnarray}
&& Prob((m_t)_{t\geq 1}) = \sum_{(w_t)_{t\geq 1}} Prob((w_t)_{t\geq 1}) \prod_{k\geq 1} p_k \mbox{ where } \nonumber \\
&& p_k = \sum_{q\geq 1} (\frac{w_k+|V|}{2^L})^{q-1}(1-\frac{w_k+|V|}{2^L}) \cdot \nonumber \\
&& \hspace{.3cm} {q \choose m_k} (1-\frac{w_k}{2^L-|V|})^{m_k} (\frac{w_k}{2^L-|V|})^{q-m_k}. \label{eqp5}
\end{eqnarray}

\vspace{.2cm}

\noindent
{\bf Expected number of blocks in $T$.}
Notice that the expectation $E[m_k|(w_t)_{t\geq 1}]$ is equal to
\begin{eqnarray*}
 && \sum_{q\geq 1} (\frac{w_k+|V|}{2^L})^{q-1}(1-\frac{w_k+|V|}{2^L})q(1-\frac{w_k}{2^L-|V|}) \\
&& =\frac{1-w_k/(2^L-|V|)}{1-(w_k+|V|)/2^L}= 1/(1-|V|/2^l).
\end{eqnarray*}
This is proved in a different way in Section \ref{sec:Chernoff}, where we use (\ref{alpha}) to show that the expectation of the usage of $T$ is at most $2n$ for utilization $N/2^L\leq 2$ and for bucket size $Z\geq 4$. 
For this reason we expect to be able to use a Chernoff bound to prove that with negligible probability  $T$'s usage is more than $T$'s capacity:

\vspace{.2cm}

\noindent
{\bf Probability generating functions.}
From (\ref{eqp1}) and (\ref{eqp5}):
\begin{eqnarray*} 
&& Prob(\sum_{t=0}^{n-2|V|} m_t>nZ+R)\leq \max_{(w_t)_{t\geq 1}} p, \mbox{ where} \\
&& p=\sum_{(m_t)_{t=0}^{n-2|V|} \mbox{ with } \sum_{t=0}^{n-2|V|} m_t>nZ+R} p_0 \cdot \prod_{k\geq 1} p_k.
\end{eqnarray*}
The probability generating function corresponding to $p_0$ is
\begin{eqnarray*}
&& \sum_{m= 0}^N {N \choose m} (\frac{|V|}{2^L})^m (1-\frac{|V|}{2^L})^{N-m} X^m \\
&& = (1+(|V|/2^L)(X-1))^N \leq exp((|V|/2^L)(X-1)N)
\end{eqnarray*}
and the probability generating function corresponding to $p_k$ is equal to
\begin{eqnarray}
&& \sum_{q\geq 1} \alpha^{q-1}(1-\alpha)  [1+\beta (X-1)]^q.\label{probpk}
\end{eqnarray}
where
$$\alpha = \frac{w_k+|V|}{2^L}\leq 1 \mbox{ and } \beta = 1-\frac{w_k}{2^L-|V|}.$$
By the binomial theorem, (\ref{probpk}) is equal to
\begin{eqnarray*}
&& \sum_{q\geq 1}  \alpha^{q-1}(1-\alpha)\sum_{m=0}^q {q \choose m} (\beta(X-1))^m \\
&=& 1+ \sum_{m\geq 1} \sum_{q\geq m} {q \choose m} \alpha^{q-1} (1-\alpha)(\beta(X-1))^m \\
&=& 1+ \sum_{m\geq 1} \frac{\alpha^{m-1}}{(1-\alpha)^m}(\beta(X-1))^m.
\end{eqnarray*}
Notice that $\alpha\leq 1$ and $\beta/(1-\alpha) = 1/(1-|V|/2^L)\leq 1/(1-N/(Z2^L))$ by (\ref{alpha}).\footnote{If we do not use the bound $\alpha \leq 1$ but explicitly maximize over all possible sequences $(w_t)_{t\geq 1}$ that may correspond to a subtree $T$ of size $n$, then we may be able to prove the main theorem for even smaller bucket sizes $Z=4$ or $Z=5$.}
This proves that (\ref{probpk}) is at most
\begin{eqnarray*}
&& 1+ \sum_{m\geq 1} \left[ \frac{(X-1)}{1-N/(Z2^L)}\right]^m \\
&=& 1+ \frac{(X-1)}{(1-N/(Z2^L))-(X-1)} \\
&\leq & exp(\frac{(X-1)}{(1-N/(Z2^L))-(X-1)})
\end{eqnarray*}
for $1\leq X < 2-N/(Z2^L)$.

The probability generating function (corresponding to $p$) of the total number of blocks $M=\sum_{k} m_k$ in $T$ ($T$'s usage) given $(w_t)_{t\geq 1}$
 is  equal to the product of the probability generating functions of $p_j$, $0\leq j\leq n-2|V|$, which is at most
$$ exp( \frac{(X-1)}{(1-N/(Z2^L))-(X-1)}(n-2|V|) + (X-1)|V|\frac{N}{2^L}).
$$
Let 
\begin{equation} L\geq \lceil \log N \rceil -1. \label{condN} \end{equation}
Then $N/2^L\leq 2$, hence, the contribution to $(X-1)|V|$ in the exponential is negative and we obtain the upper bound
$$ exp( \frac{(X-1)}{(1-N/(Z2^L))-(X-1)}n).$$
Let $M[X]$ denote this function.


\vspace{.2cm}

\noindent
{\bf Markov's inequality.}
By Markov's inequality, $\forall z$ with 
\begin{equation}
1< e^z<2-N/(Z2^L), \label{cons}
\end{equation}
 the tail distribution of the total number of blocks $M$ in $T$ given $(w_t)_{t\geq 1}$ is upper bounded by
\begin{eqnarray} 
Prob(M\geq nZ+R) &=& Prob(e^{zM}\geq e^{z(nZ+R)}) \nonumber \\
&\leq& \frac{E[e^{zM}]}{e^{z(nZ+R)}}  =\frac{M[e^z]}{e^{z(nZ+R)}}. \nonumber
\label{eq3} 
\end{eqnarray}
Since the upper bound is independent of $(w_t)_{t\geq 1}$, it holds for the total number of blocks in $T$ without a condition on 
$(w_t)_{t\geq 1}$, i.e.,
\begin{eqnarray*} 
&& Prob(u({\cal R}_L(Z)[\mbox{{\bf s}}];T)> nZ+R|a(\mbox{{\bf s}})=\mbox{{\bf a}})\leq \frac{M[e^z]}{e^{z(nZ+R)}} \\
&& = exp(n\left[ \frac{e^z-1}{2-N/(Z2^L)-e^z} - zZ\right] -zR ). 
%\nonumber %\label{eqUM}
\end{eqnarray*}

\vspace{.2cm}

\noindent
{\bf Main theorem.}
The first part of the main theorem follows by substituting $Z=7$, $e^z=1.6$ and bounding $L\geq \lceil \log N \rceil +1$ (notice that both (\ref{condN}) and (\ref{cons}) hold), which gives $0.625^R/4.3^n$ as an upper bound on the tail distribution.
Plugging this into the union bound (\ref{equnion}) 
yields
\begin{eqnarray}
&& Prob(u({\cal T}_L(Z)[\mbox{{\bf s}}])>R|a(\mbox{{\bf s}})=\mbox{{\bf a}}) \nonumber \\
&& \leq \sum_{n\geq 1} 4^n 0.625^R/4.3^n \leq 14\cdot 0.625^R. \label{eqmain}
\end{eqnarray}
By substituting $Z=6$, $e^z=1.5$ and bounding $L\geq \lceil \log N \rceil +3$ we obtain the bound $370\cdot 0.667^R$, the second part of the main theorem.




==> ORAManalysisShort.tex <==



\section{Theoretic Bounds}\label{sec:fail}

In this section we will bound the probability that, after a sequence of load/store operations, non-recursive Path-ORAM exceeds its stash size: We will show that this probability decreases exponentially in the size of the stash for a {\em constant} bucket size.

By ${\cal T}_L(Z)$ we denote a non-recursive Path-ORAM with $L+1$ levels in which each bucket stores $Z$ real/dummy blocks; the root is at level $0$ and the leafs are at level $L$. 

We define a {\em sequence of load/store operations} $\mbox{{\bf s}}$ as a triple $(\mbox{{\bf a}},\mbox{{\bf x}}, \mbox{{\bf y}})$ that contains (1) the sequence $\mbox{{\bf a}}=(a_j)_{j=1}^s$ of block addresses of blocks that are loaded/stored, (2) the sequence of labels $\mbox{{\bf x}}=(X_j)_{j=1}^s$ as seen by the server, and (3) the sequence $\mbox{{\bf y}}=(Y_j)_{j= 1}^s$ of remapped leaf labels. $(a_1,Y_1,X_1)$ corresponds to the most recent load/store operation, $(a_2,Y_2,X_2)$ corresponds to the next most recent load/store operation, etc. The number of load/store operations is denoted by $s=|\mbox{{\bf s}}|$. The {\em working set} corresponding to $\mbox{{\bf a}}$ is defined as the number of distinct block addresses $a_j$ in $\mbox{{\bf a}}$. We write $a(\mbox{{\bf s}})=\mbox{{\bf a}}$.

By ${\cal T}_L(Z)[\mbox{{\bf s}}]$ we denote the distribution of real blocks in ${\cal T}_L(z)$ after a sequence $\mbox{{\bf s}}$ of load/store operations starting with an empty ORAM; $\mbox{{\bf s}}$ completely defines all the randomness needed to determine, for each block address $a$, its leaf label and which bucket/stash stores the block that corresponds to $a$. In particular the {\em number} of real blocks  stored in the buckets/stash can be reconstructed. 

We assume an infinite stash and in our analysis we investigate the usage $u({\cal T}_L(Z)[\mbox{{\bf s}}])$ of the stash defined as the number of real blocks that are stored in the stash after a sequence $\mbox{{\bf s}}$ of load/store operations.  In practice the stash is limited to some size $R$ and Path-ORAM fails after a sequence $\mbox{{\bf s}}$ of load/store operations if the stash needs more space: this happens if and only if the usage of the infinite stash is at least $u({\cal T}_L(Z)[\mbox{{\bf s}}])>R$.

\begin{theorem}[Main] 
Let $\mbox{{\bf a}}$ be any sequence of block addresses with a working set of size at most $N$.
For a bucket size $Z=7$, tree depth $L\geq \lceil \log N \rceil +1$ and stash size $R$, the probability of a Path ORAM failure after a sequence of load/store operations corresponding to $\mbox{{\bf a}}$, is at most 
\begin{eqnarray*}
&& Prob(u({\cal T}_L(Z)[\mbox{{\bf s}}])>R|a(\mbox{{\bf s}})=\mbox{{\bf a}}) \leq 14\cdot 0.625^R,
\end{eqnarray*}
where the probability is over the coin flips that determine $\mbox{{\bf x}}$ and $\mbox{{\bf y}}$ in $\mbox{{\bf s}}=(\mbox{{\bf a}},\mbox{{\bf x}}, \mbox{{\bf y}})$.

For $Z=6$ and $L\geq \lceil \log N \rceil +3$ we obtain the bound $370\cdot 0.667^R$.
\label{thm:main}
\end{theorem}

As a corollary,  for $s$ load/store operations on $N$ data blocks, Path ORAM with client storage $\leq R$ blocks, server storage $28N$ blocks and bandwidth $14\log N$ blocks per load/store operation, fails during one of the $s$ load/store operations with probability $\leq s\cdot 14\cdot 0.625^R$. 
So, if we assume the number of load/stores is equal to $s=poly(N)$, then, 
for a stash of size $O(\log N)\omega(1)$, the probability of Path ORAM failure during one of the load/store operations is negligible in $N$. 


\vspace{.2cm}

\noindent
{\bf Proof outline.}
The proof of the main theorem consists of several steps: First, we introduce a second ORAM, called $\infty$-ORAM, together with an algorithm that post-processes the stash and buckets of $\infty$-ORAM in such a way that if $\infty$-ORAM gets accessed by a sequence $\mbox{{\bf s}}$ of load/store operations, then post-processing leads to a distribution of real blocks over buckets that is exactly the same as the distribution as in Path ORAM after being accessed by $\mbox{{\bf s}}$. 

Second, we characterize the distributions of real blocks over buckets in (a not post-processed) $\infty$-ORAM for which post-processing leads to a stash usage $>R$. We show that the stash usage after post-processing is $>R$ if and only if there exists a subtree $T$ for which its "usage" in $\infty$-ORAM is more than its "capacity". This means that we can use the union bound to upper bound $Prob({\cal T}_L(Z)[u(\mbox{{\bf s}})]>R|a(\mbox{{\bf s}})=\mbox{{\bf a }})$ as a sum of probabilities over subtrees.

Third, we analyze the usage of subtrees $T$. We show how a mixture of a binomial and a geometric probability distribution expresses the probability of the number of real blocks that do not get evicted from $T$ after a sequence $\mbox{{\bf s}}$ of load/store operations. By using the Chernoff bounding technique we prove the main theorem.


\vspace{-1mm}
\subsection{$\infty$-ORAM} \label{infty-oram}

We define $\infty$-ORAM, denoted by ${\cal R}_L(Z)$, as an ORAM that exhibits the same tree structure as Path-ORAM with $L+1$ levels but where each bucket has an {\em infinite} size. The interface of ${\cal R}_L(Z)$ operates as the interface of ${\cal T}_L(\infty)$ with the following distinguishing exception: 
Each bucket in ${\cal R}_L(Z)$  is partially stored in server storage and partially stored in the ORAM stash at the client; $Z$ indicates the maximum number of blocks in a bucket that can be stored in server storage. If a bucket  has more than $Z$ real blocks, then the additional blocks are stored in the $\infty$-ORAM stash. 

We define {\em post-processing}\footnote{Notice that the post-processing allows us to reason about Path-ORAM's stash size. It does not hide memory access patterns: $\infty$-ORAM + post-processing is only a tool for analysis, it is not an ORAM algorithm in itself.} $G({\cal R}_L(Z)[\mbox{{\bf s}}])$ as a Greedy algorithm $G$ that takes as input the state of ${\cal R}_L(Z)$ after a sequence $\mbox{{\bf s}}$ of load/store operations and repeats the following strategy:
\vspace{-1mm}
\begin{enumerate}
\item Select a block in the stash that was not selected before. Suppose it has leaf label $L$ and is stored in the bucket at level $h$ on the path from the root to leaf $L$. 
\emil{Overloading of terminology $L$.}
\vspace{-3mm}
\item Find the highest level $i\leq h$ such that the bucket at level $i$ on the path to leaf $L$ stores $<Z$ blocks. 
If such a bucket exists, then use it to store the block. If it does not exist, then leave the block in the stash. 
\end{enumerate}

\begin{lemma} \label{lem1} The stash usage in a post-processed $\infty$-ORAM is exactly the same as the stash usage in Path-ORAM:
\vspace{-1mm}
$$ u(G({\cal R}_L(Z)[\mbox{{\bf s}}])) = u({\cal T}_L(Z)[\mbox{{\bf s}}]).$$
\end{lemma}

\vspace{-2mm}
\noindent
{\em Proof:} We first notice that the order
 in which the Greedy strategy $G$ processes blocks from the stash does not affect the number of real blocks in each bucket that are stored  in server storage after post-processing: 
Suppose the Greedy strategy first processes a stash block $b_1$ with label $X_1$ stored in a bucket at level $h_1$ and suppose it finds empty space in server storage at level $i_1$; the Greedy strategy up to block $b_1$ has used up all the empty space in server storage allocated to the buckets along the path to the leaf with label $X_1$ at levels $i_1<i\leq h_1$. Suppose next a stash block $b_2$ with label $X_2$ stored in a bucket at level $h_2$ finds empty space in server storage at level $i_2$; the Greedy strategy up to block $b_2$, which includes the post-processing of $b_1$, has used up all the empty space in server storage allocated to the buckets along the path to the leaf with label $X_2$ at levels $i_2<i\leq h_2$.  If we swap the post-processing of $b_1$ and $b_2$, then $b_2$ is able to find empty space in the bucket at level $i_2$, but may find empty space at a higher level since $b_1$ has not yet been processed. In this case, $i_2<i_1$ and paths $X_1$ and $X_2$ intersect at least up to and including level $i_1$. This means that $b_2$ is stored at level $i_1$ and $b_1$ will use the empty space in server storage at level $i_2$. This means that the number of blocks that are stored in the different buckets after post-processing $b_1$ and $b_2$ is the same if $b_1$ is processed before or after $b_2$.

Now, we are able to show, by using induction in $|\mbox{{\bf s}}|$, that
for each bucket $b$ in a post-processed $\infty$-ORAM after a sequence $\mbox{{\bf s}}$ of load/store operations, the number of real blocks stored in $b$ that are in server storage is equal to the number of blocks stored in the equivalent bucket in Path-ORAM after applying the same sequence $\mbox{{\bf s}}$ of load/store operations: The statement clearly holds for $|\mbox{{\bf s}}|=0$ when both ORAMs are empty. Suppose it holds for $|\mbox{{\bf s}}|\geq 0$. Consider the next load/store operation to some leaf $L'$. After reading the path to leaf $L'$ into the cache, Path-ORAM moves blocks from its cache/stash into the path from root to leaf $L'$ according to algorithm $G(.)$. Therefore, postprocessing after the first $|\mbox{{\bf s}}|$ operations followed by the Greedy approach of Path ORAM that processes the  $(|\mbox{{\bf s}}|+1)$-th operation is equivalent to post-processing after $|\mbox{{\bf s}}|+1$ operations where some blocks may be post-processed twice. Since the order in which blocks are post-processed does not matter, we may group together the multiple times a block $b$ is being post-processed and this is equivalent to post-processing $b$ exactly once as in $G(.)$. The number of real blocks in the stash is the same and this proves the lemma.

\vspace{-1mm}
\subsection{Usage/Capacity Bounds} \label{failure}

To investigate which distributions of real blocks over buckets in a not post-processed $\infty$-ORAM ${\cal R}_L(Z)$ lead to a stash usage of $>R$ after post-processing, we start by analyzing distributions of blocks over subtrees: 
When we talk about a subtree $T$, we always implicitly assume that it is rooted at the root of the ORAM tree, i.e., $T$ contains the root of the ORAM tree and all its nodes are connected to this root.
We define $n(T)$ to be the total number of nodes in $T$.
For $\infty$-ORAM we define the usage $u({\cal R}_L(Z)[\mbox{{\bf s}}];T)$ of $T$ after a sequence $\mbox{{\bf s}}$ of load/store operations as the actual number of real blocks that are stored in the buckets of $T$ (in $\infty$-ORAM blocks in a bucket are either in server storage or in the stash).

The following lemma characterizes the stash usage:

\begin{lemma} \label{lem2}
The stash usage $u(G({\cal R}_L(Z)[\mbox{{\bf s}}]))$ in post-processed $\infty$-ORAM is $> R$ if and only if there exists a subtree $T$ in ${\cal R}_L(Z)$ such that $u({\cal R}_L(Z)[\mbox{{\bf s}}];T)> n(T)Z+R.$
\end{lemma}

\noindent
{\em Proof:} For a stash of size $R$, since post-processing can at most store $n(T)Z$ real blocks in $T$ in server storage,
we may interpret $n(T)Z+R$ as the {\em capacity} of $T$. Clearly, if the usage of $T$ is more than the capacity of $T$, then post-processing leads to a stash usage of $>R$.

Suppose that $u(G({\cal R}_L(Z)[\mbox{{\bf s}}]))>R$. Define $T$ as the union of all paths  from the root to a bucket $b$ for which the buckets along the path in $G({\cal R}_L(Z)[\mbox{{\bf s}}])$ each have $Z$ real blocks stored in server storage. Then, $u(G({\cal R}_L(Z)[\mbox{{\bf s}}]);T)>n(T)Z+R$. Also, if a real block in $T$ or in the stash originated from a bucket $b$, then the Greedy approach of post-processing implies that the buckets on the path from where the block is stored in T to bucket $b$ each store $Z$ real blocks, therefore, $b\in T$. This shows that $u({\cal R}_L(Z)[\mbox{{\bf s}}];T)\geq u(G({\cal R}_L(Z)[\mbox{{\bf s}}]);T)$, which finishes the proof of the lemma.

Let $\mbox{{\bf a}}$ be a sequence of block addresses.
As a corollary to Lemmas \ref{lem1} and \ref{lem2}, we obtain
\begin{eqnarray*}
&& Prob(u({\cal T}_L(Z)[\mbox{{\bf s}}])>R|a(\mbox{{\bf s}})=\mbox{{\bf a}}) \\
&=& Prob(u(G({\cal R}_L(Z)[\mbox{{\bf s}}]))> R|a(\mbox{{\bf s}})=\mbox{{\bf a}}) \\
&=& Prob( \exists_T \ u({\cal R}_L(Z)[\mbox{{\bf s}}];T)> n(T)Z+R|a(\mbox{{\bf s}})=\mbox{{\bf a}})\\
&\leq& \sum_T Prob(u({\cal R}_L(Z)[\mbox{{\bf s}}];T)> n(T)Z+R|a(\mbox{{\bf s}})=\mbox{{\bf a}}),
\end{eqnarray*}
where the inequality follows from the union bound. The probabilities are over the coin flips that determines $\mbox{{\bf s}}$ given $a(\mbox{{\bf s}})=\mbox{{\bf a}}$.

Since the number of ordered binary trees of size $n$ is equal to the Catalan number $C_n$, which is $\leq 4^n$,
\begin{eqnarray}
&& Prob(u({\cal T}_L(Z)[\mbox{{\bf s}}])>R|a(\mbox{{\bf s}})=\mbox{{\bf a}}) \leq  \label{equnion} \\
&& \sum_{n\geq 1} 4^n \max_{T:n(T)=n} Prob(u({\cal R}_L(Z)[\mbox{{\bf s}}];T)> nZ+R|a(\mbox{{\bf s}})=\mbox{{\bf a}}). \nonumber 
\end{eqnarray}


\subsection{Chernoff Bound}\label{sec:Chernoff}

We will upper bound the probability in the sum of the right-hand side of (\ref{equnion}) for $T$ with $n(T)=n$. To this purpose
let $\mbox{{\bf a}}=(a_j)_{j=1}^s$ be a sequence of block addresses with working set size $N$, i.e., $\mbox{{\bf a}}$ has $N$ different block addresses.  Let $\mbox{{\bf s}}=(\mbox{{\bf a}},\mbox{{\bf y}}=(Y_j)_{j=1}^s,\mbox{{\bf x}}=(X_j)_{j=1}^s)$ be a sequence of load/store operations. In this section we only provide a proof sketch, precise arguments are in Section~\ref{app:Chernoff}.

For each block $Y_j$ we wish to determine the probability that $Y_j$ gets evicted from $T$.  
We first observe that $Y_j$ never gets evicted if  $Y_j\in V$, the set of  leafs in $T$ that are also leafs in the ORAM tree.  Therefore, the expectation of the usage of $T$ is at most
\begin{eqnarray*}
&& E[u({\cal R}_L(Z)[\mbox{{\bf s}}];T)|a(\mbox{{\bf s}})=\mbox{{\bf a}}] \leq \\
&& E[\# Y_j \in V] + E[u({\cal R}_L(Z)[\mbox{{\bf s}}];T)|a(\mbox{{\bf s}})=\mbox{{\bf a}},\forall_j Y_j\not\in V].
\end{eqnarray*}
Since the probability that $Y_j\in V$ is equal to $|V|/2^L$, 
\begin{equation} E[\# Y_j \in V]=N|V|/2^L.\label{c0} \end{equation}

Next we observe that $Y_j$ can only get evicted over paths to leafs with labels $X_j, X_{j-1},\ldots, X_1$ (which correspond to the more recent load/store operations).  Let $u_j$, as a function of the label values for $X_j, X_{j-1},\ldots, X_1$, be the probability that $Y_j$ is evicted from $T$ given $Y_j\not\in V$. In $\infty$-ORAM the worst-case address pattern $\mbox{{\bf a}}$ for a fixed working set size $N$ does not duplicate block addresses, i.e., $s=N$ and as a consequence the labels in $(X_j)_{j=1}^N$ and $(Y_j)_{j=1}^N$  are all statistically independent of one another: Assuming non-duplicated block addresses, $u_1\leq u_2\leq u_3 \leq \ldots$, hence, there exist segments $U_1 = \{1,2,\ldots, q_1\}\neq \emptyset$, $U_2=\{q_1+1, \ldots, q_1+q_2\}\neq \emptyset$, $\ldots$, such that within each segment $U_k$ the probabilities $u_j$, $j\in U_k$, are all equal to one another. I.e, there exists a probability $h_k$ such that $h_k=u_j$, $j\in U_k$. We notice that the number of segments $U_k$ with $h_k<1$ equals $n-2|V|$, the number of buckets that are one edge away from $T$, minus 1. By the definition of $h_k$,
\begin{equation} E[\# Y_j, j\in U_k, \mbox{ not evicted from } T \ | \ |U_k|] = (1-h_k)|U_k|.\label{c1} \end{equation}

We notice that $u_{j+1}\neq u_{j}$ if and only if $X_{j+1}$ matters in the calculation of $u_{j+1}$, i.e., there exists a block that can get evicted from $T$ over the path to the leaf with label  $X_{j+1}$ while it cannot get evicted over a path  to a 
leaf with label $X_i$, $1\leq i\leq j$. This means that 
$X_{j+1}\not\in V$ and, for each $1\leq i\leq j$, the intersection of the path to $X_{j+1}$ and the path to $X_i$ lies inside $T$, i.e., a block with label $X_{j+1}$ cannot get evicted from $T$ over a path to leaf $X_i$.
This proves
\begin{eqnarray*}
&& Prob(X_{j+1} \mbox{ such that } u_{j+1} = u_j) \\
&=& Prob(X_{j+1} \in V \mbox{ or } \\
&& \hspace{0.5cm} X_{j+1} \mbox{ can be evicted from } T \mbox{ over } (X_i)_{i=1}^j) \\
&=& Prob(X_{j+1} \mbox{ evicted from } T | X_{j+1}\not\in V)Prob(X_{j+1}\not\in V) \\
&& + Prob(X_{j+1}\in V)\\
&=& u_j (1-|V|/2^L) + |V|/2^L \\
&=& 1-(1-u_j)(1-|V|/2^L).
\end{eqnarray*}
This shows that $|U_k|$ has a geometric distribution with expectation $E[|U_k|]$ equal to
\begin{eqnarray}  && \sum_{q\geq 1} (1-(1-h_k) (1-|V|/2^L))^{q-1} (1-h_k) (1-|V|/2^L) q  \nonumber \\
&& = \frac{1}{(1-h_k) (1-|V|/2^L)}.\label{c2} \end{eqnarray}

Combining (\ref{c1}) and (\ref{c2}) yields
\begin{eqnarray*}
&& E[u({\cal R}_L(Z)[\mbox{{\bf s}}];T)|a(\mbox{{\bf s}})=\mbox{{\bf a}},\forall_j Y_j\not\in V] \\
&& \leq \sum_{k=1}^{n-2|V|} \frac{1-h_k}{(1-h_k) (1-|V|/2^L)} = \frac{n-2|V|}{1-|V|/2^L}.
\end{eqnarray*}
Together with (\ref{c0}), the expectation of the usage of $T$ is at most 
$N|V|/2^L+(n-2|V|)/(1-|V|/2^L)$.

In (\ref{equnion}) we are only interested in a non-zero probability that $T$'s usage is $>nZ+R$. Therefore, since $|V|\leq n$ and $T$'s usage is at most $N$, we may constrain $|V|\leq N/Z$.
For $N/2^L\leq 2$ and $Z\geq 4$,
 the expectation is at most $n/(1-|V|/2^L)\leq 2n$. In the sum of the right-hand side of (\ref{equnion}) we bound the probability that $T$'s usage is $>nZ+R$, which is a multiple larger than the expectation of the usage in $T$. This means that we are able to apply a Chernoff bounding technique to prove the main theorem: For bucket size $Z$ large enough, we are able to compensate the $4^n$ term in (\ref{equnion}).




\input{Chernoff}













==> StashSizeProofOverview.tex <==
\section{Proof of Logarithmic Stash Size}
\label{sec:StashSizeProof}
\emil{Proof overview goes here. Reference the full online version.}

==> extensions.tex <==
\emil{move integrity back here}


\section{Extensions and Optimizations}
\emil{talk about caching levels of the tree}


\subsection{Delayed Writes}
\emil{Say that this idea was introduced in prior work.}

Writes (eviction from data in the stash) does not have to be done at the end of every access as described in Figure~\ref{fig:Access}. Instead, writes can done in the background or they can even be delayed for when the client is more idle. Writes cannot be delayed indefinitely because the stash size will keep growing until the writes complete.

